Differentiable Electron Microscopy Simulation: Methods and Applications for Visualization

We propose a new microscopy simulation system that can depict atomistic models in a micrograph visual style, similar to results of physical electron microscopy imaging. This system is scalable, able to represent simulation of electron microscopy of tens of viral particles and synthesizes the image faster than previous methods. On top of that, the simulator is differentiable, both its deterministic as well as stochastic stages that form signal and noise representations in the micrograph. This notable property has the capability for solving inverse problems by means of optimization and thus allows for generation of microscopy simulations using the parameter settings estimated from real data. We demonstrate this learning capability through two applications: (1) estimating the parameters of the modulation transfer function defining the detector properties of the simulated and real micrographs, and (2) denoising the real data based on parameters trained from the simulated examples. While current simulators do not support any parameter estimation due to their forward design, we show that the results obtained using estimated parameters are very similar to the results of real micrographs. Additionally, we evaluate the denoising capabilities of our approach and show that the results showed an improvement over state-of-the-art methods. Denoised micrographs exhibit less noise in the tilt-series tomography reconstructions, ultimately reducing the visual dominance of noise in direct volume rendering of microscopy tomograms.

==> includes/experiments-and-use-case.tex <==
To accellerate the performance of the TEM simulator we have developed the GPU-TEM simulator that exploits parallelism of the GPU hardware using the CUDA API~\cite{cuda}. Currently, a large portion of the simulator pipeline is implemented in CUDA, while there are still few pipeline stages where we resort to pure GPU implementation. [TODO which stage is parallelized and which is not?]

We confront the original TEM-simulator with the current GPU version, which already shows substantial benefits for large scenes representing realistic microscopy-experiment scenario. 

We use Pytorch~\cite{paszke2019pytorch} and Taichi~\cite{hu2018taichi} to implement our \gls*{difftem} simulator. 

\subsection{Performance evaluation}
We compared the performance of the original TEM simulator and our GPU-TEM. In the phantom generator we used the model of SARS-CoV-2 virus modelled by Nguyen~\etal~\cite{nguyen2021modeling}, ZIKA virus \gls*{pdb}id 5IRE and \gls*{tmv} PDBid 2OM3. The details of each model are shown in~\autoref{table:desc_virus_model}. All performance experiments were done on a Windows system with one processor Intel(R) Xeon(R) CPU E5-2687W v4 3GHz and one GPU NVIDIA GeForece RTX 3090.

\begin{table}[H]
\small
\caption{Details of the models used in the performance evaluation.}
\label{table:desc_virus_model}
\centering
\begin{tabular}{lccc}
\toprule
\textsc{Virions}& \textsc{No. of pdbs} & \textsc{No. of atoms}  \\ 
\midrule
{\gls*{tmv}} & {1} & {12505} \\ 
{ZIKA} & {1} & {21149} \\
{SARS-CoV-2} & {17} & {$\approx 13$ millions} \\ 
\bottomrule
\end{tabular}
\end{table}

\subsection{MTF parameters estimation}
For estimating \gls*{mtf} parameters, we performed experiments on both synthetic and real data. The synthetic data is created from the envelope of SARS-CoV-2 virion and \gls*{tmv} virion. The real dataset is provided by Yao~\etal~\cite{Sai2020:CryoET-Pipeline} consists of 20 tilt series containing several SARS-CoV-2 virions each, but we only use cropped sub-image containing background for optimization. The real data was acquired using a Titan Krios microscope with K3 detector from Gatan, operated at a voltage of $300$ kV. 
The ground truth of \gls*{mtf} parameters for real data was obtained by performing curve-fitting from \gls*{mtf} curve of Gatan K3 detector\footnote{https://www.gatan.com/K3\#resources}. The ground truth values of \gls*{mtf} parameters for synthetic data \gls*{tmv} virion is provided by Rullg{\aa}rd~\etal~\cite{rullgaard2011simulation} in their simulation and calibrated with their real data which is the micrograph of \gls*{tmv} virions measured by a Philips CM 200 FEG \gls*{tem} microscope. We conducted experiments for each loss function (\gls*{mse}, \gls*{mse} + \gls*{ffl}) with different number of background images of synthetic data to see the correlation between performance of each loss and number of images. Then we conducted the experiments on the real data with the number of images similar to the number that gives the best performance on synthetic data. We also conducted experiments with different \gls*{ffl} loss $\alpha$ values:  $(0.0, 0.5, 1.0, 2.0)$. Beside, to demonstrate the generalization of the estimation method, we also experimented with synthetic \gls*{mtf} that has the shape is different with real \gls*{mtf}.
All estimating \gls*{mtf} parameters experiments were conducted on Linux system with four GPUs NVIDIA RTX A6000.

\subsection{Denoising}
First, we conducted experiments using a synthetic dataset generated with our simulator given an atomistic model (\ie, \gls*{tmv} model from the research by Sachse \etal~\cite{SACHSE2007812}). In this setting, we obtain a clean ground truth data that are synthesized by bypassing the quantization. 

In simulation and in real electron microscopy process, the dose, measured in electrons per nm\textsuperscript{2} per projection, is a major factor that determines \gls*{snr}. We tested our denoising method with synthetic datasets with applying varying doses. The higher the dose is, the higher \gls*{snr} is. For generating a tilt series of 60 projections, 100 electrons/nm\textsuperscript{2} per projection is a typical low dose while 200 is a typical high dose. We tested datasets of doses \{100, 200, 300, 500, 700, 1000, 1500, 2000\} because it is possible to use a very high dose (\eg, 1000) if the number of total projections is low and thus the total dose stays the same. Moreover, the number of available projections of the same scene (\ie, same tilt angle and specimen) also affects denoising quality. We tested our method on the numbers of available projections of \{2, 5, 10, 25, 50\}. We denote varying data settings with pairs, i.e., dose, the number of available projections.

To compare with the original Noise2Noise~\cite{noise2noise} model and \topaz~\cite{topaz_denoiser}, we trained a Noise2Noise model and a \topaz~model with our synthetic data. The data setting for training Noise2Noise model is (100, 5000) while it is (100, 4500) for training \topaz~model. We also use pretrained \topaz~model to contrast the results.


In the experiments using real micrographs, we use the tilt series from Yao \etal~\cite{Sai2020:CryoET-Pipeline}, which is SARS-CoV-2. The dose in their data collection is 320 electrons/nm\textsuperscript{2} per projection. Therefore, without data augmentations, the setting is (320, 1). As discussed in Section~\ref{denoising_section}, our method cannot work in a scenario with only single projection, so in our experiments, we apply a number of data augmentations. In the setting \texttt{Ours(T)}, the data augmentation with Topaz P is used, yielding one more projection, which means the setting is (320, 2). In the setting denoted as \texttt{Ours(N)}, neighboring projections of a projection are aligned and used, so the data setting is (320, 3). In the setting \texttt{Ours(T+N)}, Topaz P and aligned neighboring projections are used, so the data setting is (320, 6). The case of \texttt{Ours(T+N)} matches exactly our \autoref{denoising_optimization} while in the case of \texttt{Ours(T)}, $P_n=\{P\}$, and in the case of \texttt{Ours(N)}, preprocessing with \topaz~is not used (\ie, $P_{train}=Normalize(P_n)$). The results of the three cases (\ie, \texttt{Ours(T)}, \texttt{Ours(N)} and \texttt{Ours(T+N)}) will be presented along with the projection preprocessed by \texttt{Topaz P} and the noisy projection in Section~\ref{denoising_real_results}.

==> includes/results-and-discussion.tex <==
We discuss the results of our work in three parts: performance of our GPU-TEM, \gls*{mtf} estimation and denoising.
\subsection{Performance}
We demonstrated the scalability of our GPU-TEM in two aspects: (1) number of atoms and (2) number of virion instances. The performance of each simulator for a single instance each virus type is shown in~\autoref{table:performance_atoms}. 

\begin{table}[H]
\small
\caption{Performance on \wrt number of atoms}
\label{table:performance_atoms}
\centering
\begin{tabular}{lccc}
\toprule
\textsc{Model} & \textsc{GPU-\gls*{tem}} & \textsc{\gls*{tem}~\cite{rullgaard2011simulation}}\\
\midrule
{\gls*{tmv}} & {4s} & {45s}\\ 
{ZIKA} & {1m46s} & {1m51s} \\ 
{SARS-CoV-2} & {} & {} \\ 
\bottomrule
\end{tabular}
\end{table}

From the~\autoref{table:performance_atoms}, the performance on single instance of ZIKA virus of our GPU-TEM is similar to the baseline~\cite{rullgaard2011simulation}, so we measured the performance on many instances of ZIKA, the results are shown in~\autoref{table:performance_instances}. 
As in~\autoref{table:performance_instances}, our GPU-TEM performs better for scenes containing high number of instances.

\begin{table}[H]
\small
\caption{Performance on many instances of ZIKA}
\label{table:performance_instances}
\centering
\begin{tabular}{lccc}
\toprule
\textsc{No. of instances} & \textsc{GPU-\gls*{tem}} & \textsc{\gls*{tem}~\cite{rullgaard2011simulation}}\\
\midrule
{1} & {\textbf{1m 46s}} & {1m 51s} \\ 
{5} & {3m 1s} & {2m 9s} \\ 
{10} & {3m 10s} & {2m 16s} \\ 
{50} & {\textbf{3m 30s}} & {3m 34s} \\ 
{100} & {3m 48s} & {2m 16s} \\ 
{500} & {\textbf{5m 42s}} & {21m 17s} \\ 
{1000} & {\textbf{6m 22s}} & {35m 27s} \\ 
{5000} & {\textbf{18m 9s}} & {4h11m } \\ 
\bottomrule
\end{tabular}
\end{table}


\subsection{MTF parameters estimation}
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{figures/Graphs.pdf}
\caption{\gls*{mtf} parameters estimation experiment results}
\label{fig:mtf_parameters_exp}
\end{center}
\end{figure*}

The effect of \gls*{mtf} is hard to see in the real \gls*{cryo-em} images because of low \gls*{snr} so we applied both ground truth \gls*{mtf} and predicted \gls*{mtf} on the noise-free image of synthetic scene and performed evaluation. The details of the synthetic data, the number of background images, and ground truth values of \gls*{mtf} parameters $(a, b, c, \alpha, \beta)$ are shown in~\autoref{table:desc_mtf_exp}.

\begin{table}[ht]
\small
\caption{Details of experiments for estimating \gls*{mtf} parameters}
\label{table:desc_mtf_exp}
\centering
\begin{tabular}{lccc}
\toprule
\textsc{Subject} & \textsc{\gls*{mtf} paramters} & \textsc{No. of images}\\ 
\midrule
{3 \gls*{tmv}} & {0.7, 0.2, 0.1, 10, 40} & {5, 10, 20, 50}\\ 
{$\approx 10$ SARS-CoV-2} & {0.6, 1.24, -0.84, 0.97, 0.97} & {48} \\ 
{Synthetic \gls*{mtf}} & {-2.86, 2.113, -0.1318, 57.288, 25.429} & {50} \\ 
\bottomrule
\end{tabular}
\end{table}

To evaluate the effect of the \gls*{mtf} on the noise-free image, we calculated the contribution of each frequency for the noise-free image and determined which frequency band yields the largest contribution by summing the magnitude for each band. The frequency ($\frac{1}{pixel}$) bands we used are $\left\{[0.0, 0.02), [0.02, 0.04), \ldots, [0.48, 0.5)\right\}$. If the predicted \gls*{mtf} aligns well with the most contributing frequency band of the ground truth \gls*{mtf}, their effects on the noise-free images are similar. We additionally calculated the mean and maximum difference of values for both images. If two \gls*{mtf} align with the ground truth \gls*{mtf} in the same degree, the better one is the \gls*{mtf} has the mean  and maximum differences values are smaller.

The correlation between the number of background images and the performance of each loss function on synthetic data is shown in \autoref{fig:mtf_parameters_exp}(a, b). \autoref{fig:mtf_parameters_exp}(a, b) shows that the \gls*{mse} performance decreases when the number of background images is greater than $10$, the gap between the predicted \gls*{mtf} and the ground truth \gls*{mtf} increases, the mean and maximum differences also increase. With $50$ background images, the images applied predicted \gls*{mtf} is blurring, and hard to see the details of each \gls*{tmv} virions. On the contrary, \gls*{ffl} performance improves when increasing the number of background images. The predicted \gls*{mtf} with $5$ background images is more aligned with the ground truth \gls*{mtf} than $10, 20$ background images. However, the gap between it the ground truth \gls*{mtf} is larger than the gap between the \gls*{mtf} estimated from $50$ background images. The image applied the predicted \gls*{mtf} with $50$ has the smallest mean and maximum differences values. The comparison of the best \gls*{mse} and \gls*{ffl} results is shown in~\autoref{fig:mtf_parameters_exp}(a, b). It is clear that \gls*{ffl} is better choice than \gls*{mse}.

We also investigated how the change of \gls*{ffl} $\alpha$ parameter affects the \gls*{mtf} estimation for different setting. The results are shown in  \autoref{fig:mtf_parameters_exp}(c, d). The best predicted \gls*{mtf} for \gls*{tmv}, SARS-CoV-2, and synthetic setting are obtained by using $\alpha = 2.0$, $\alpha = 0.5$, $\alpha = 2.0$, for \gls*{ffl} respectively. The best $\alpha$ value for each experiment is different because of the settings (electron dose, sample preparation, etc.) of different experiments are not the same, the distribution of frequencies in background images is changed. The results show that our system works effectively for different types of \gls*{mtf} curve. The first type is the real \gls*{mtf} (\gls*{tmv} and SARS-CoV-2) gives high modulation in the most contributing frequency band, so the details of virions are not blurry too much. The second type is the synthetic \gls*{mtf}, the modulation decreases in the most contributing frequency band, so the image is applied the \gls*{mtf} is more blurry.
Our predicted \gls*{mtf} for each case is aligned well with the ground truth in the most contributing frequency band, and give the similar effect on the noise free image. 

\subsection{Denoising}
We compare the denoising capabilities of our approach in synthetic and real settings qualitatively and quantitatively.

%\subsubsection{Synthetic Setting}
\label{sec:denoising_synth_discussion}

\begin{figure}[H]
\begin{center}
\includegraphics[trim={3.5cm 0 3.5cm 0},clip=true,width=\linewidth]{figures/denoising_imgs/synthetic/comparison_ref_sample_num=2_dose=100_normalized_metrics.png}
\caption{Denoised result comparison of synthetic data setting (100, 2)}
\label{num_2_dose_100}
\end{center}
\end{figure}

Using a synthetic data with ground truth in the setting (100, 2)~, we have very limited amount of projections (\ie, only 2) and a low dose which leads to a low \gls*{snr}. In settings like this where data are scarce and full of noise, a natural choice is to average the two available projections. Although the denoised result is not close to the noise-free reference, our method outperforms the simple average of the two available projections in terms of \gls*{ssim}~\cite{ssim}, \gls*{mse}, \gls*{psnr} and \gls*{ffl}. In the case of very high doses (\ie, {700, 1000, 1500, 2000}), we show consistently better results than simple averaging in terms of \gls*{ffl}. For example, Fig.~\ref{num_50_dose_2000} shows that the \gls*{ffl} of our method is roughly 4 times better than simple averaging. The quantitative comparisons of these two figures show that our physics-based Noise2Noise-like model is effective.

\begin{figure}[H]
\begin{center}
\includegraphics[trim={3.5cm 0 3.5cm 0},clip=true,width=\linewidth]{figures/denoising_imgs/synthetic/comparison_ref_sample_num=50_dose=2000_normalized_metrics_unavg.png}
\caption{Denoised result comparison of synthetic data setting (2000, 50)}
\label{num_50_dose_2000}
\end{center}
\end{figure}

To compare with the original Noise2Noise~\cite{noise2noise} model and \topaz~\cite{topaz_denoiser}, we present the our result of the setting (100, 50) denoted as Ours-50 in \autoref{synthetic_denoising_comparison}, in which the results of a trained Noise2Noise model, Topaz P and Topaz T are also shown. The Noise2Noise model cannot work even if we have a large amount of data available (\ie, 5000). Therefore, we further tested the performance of Topaz models with our synthetic dataset. As we can see, the pretrained model (\ie, \verb|Topaz P|) generalizes well in that it filters out high-frequency noise and preserves the particles, but it is worse than our method because the boundaries of particles are blurred. Our trained Topaz model (\ie, \verb|Topaz T|) is better in that it filters out most of noise and recognizes the positions of the particles. However, it does not preserve the shape of the particles, which makes it unusable. On the contrary, our method can work in the setting with less data (\ie, (100, 50)), which shows that our method is advantageous over training a Noise2Noise~\cite{noise2noise} model and a \topaz~\cite{topaz_denoiser} model from scratch.

It is noteworthy that the Noise2Noise model and \verb|Topaz T| are trained with data settings (100, 5000) and (100, 4500) respectively. It is not realistic nor viable to obtain such large datasets in real-world scenarios, which means these two models are not usable. However, \verb|Topaz P| generalizes well in our setting, so we will use it to do data augmentation in the real-world scenario to generate more data for our denoising method.

For more results of our method under synthetic settings, we refer the reader to the \fl{our supplementary materials}.

\begin{figure}[H]
\begin{center}
\includegraphics[width=\linewidth]{figures/denoising_imgs/synthetic/Synthetic-comparison-3.png}
\caption{Comparison of denoising the synthetic data: images in the top row show original noisy projection (NP) and clean projection (GT), in bottom row are denosing results using Trained Noise2Noise result (Noise2Noise), pretrained Topaz Denoise (Topaz P), and Topaz Denoise trained on our images (Topaz T).}
\label{synthetic_denoising_comparison}
\end{center}
\end{figure}



%\subsubsection{Real Setting}
\label{denoising_real_results}

In the setting of using the real data, we do not have noise-free ground truth projections to compare against to, so we first present results for qualitative comparisons.

\begin{figure}[H]
\begin{center}
\includegraphics[width=\linewidth]{figures/denoising_imgs/real_data_compare/RealDataDenoising.png}
\caption{Topaz: the real projection preprocessed by Topaz P; Noisy: the real noisy projection; Top: full views; Bottom: Zoom-in}
\label{denoising_with_real_data}
\end{center}
\end{figure}

\begin{table*}[t]
\centering\caption{SSIM, PSNR and FFL comparison} \label{SSIM_PSNR_FFL_comparison}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc|ccccc|ccccc}
\multicolumn{6}{c}{\textbf{SSIM}} & \multicolumn{5}{c}{\textbf{PSNR}} & \multicolumn{5}{c}{\textbf{FFL}}\\
\toprule
\multicolumn{1}{c}{}      & Noisy    & Topaz    & Ours (T)        & Ours (N)         & Ours (T+N)      & Noisy    & Topaz    & Ours (T)        & Ours (N)        & Ours (T+N)      & Noisy    & Topaz    & Ours (T)        & Ours (N)   & Ours (T+N)      \\
\midrule
\multicolumn{1}{r|}{Noisy} & 1.0000   & 0.6017   & 0.4139   & 0.7395   & \textbf{0.6547}   & 361.200  & 65.8250  & 65.8270  & 70.1500  & \textbf{66.1000}  & 0.0000   & 0.0096   & 0.0082   & 0.0032   & \textbf{0.0095}   \\
\multicolumn{1}{r|}{Topaz} & 0.6017   & 1.0000   & 0.6894   & 0.7184   & \textbf{0.8651}   & 65.8250  & 361.200  & 72.2000  & 68.9700  & \textbf{75.0400}  & 0.0096   & 0.0000   & 0.0012   & 0.0045   & \textbf{0.0008}   \\
\multicolumn{1}{r|}{Ours (T)}     & 0.4139   & 0.6894   & 1.0000   & 0.7797   & 0.8001   & 65.8270  & 72.2000  & 361.200  & 71.6200  & 76.2800  & 0.0082   & 0.0012   & 0.0000   & 0.0020   & 0.0001   \\
\multicolumn{1}{r|}{Ours (N)}     & 0.7395   & 0.7184   & 0.7797   & 1.0000   & 0.9098   & 70.1500  & 68.9700  & 71.6200  & 361.200  & 71.6700  & 0.0032   & 0.0045   & 0.0020   & 0.0000   & 0.0029   \\
\multicolumn{1}{r|}{Ours (T+N)}   & 0.6547   & 0.8651   & 0.8001   & 0.9098   & 1.0000   & 66.1000  & 75.0400  & 76.2800  & 71.6700  & 361.200  & 0.0095   & 0.0008   & 0.0001   & 0.0029   & 0.0000   \\
\bottomrule
\end{tabular}
}
\end{table*}
In \autoref{denoising_with_real_data}, we can see \verb|Topaz| has block-like artifacts and \verb|Noisy| contains more noise while the other techniques have few differences. However, if we zoom-in the images, as shown in the bottom of ~\autoref{denoising_with_real_data}, we can see (1) \verb|Topaz| has more blurring artifacts, (2) \verb|Noisy| has the most noise, and (3) \verb|T+N| is better than \verb|N| and \verb|T| in that it has less high-frequency noise while preserving clear boundaries. This makes our method \verb|T+N| the best among these five because of its good balance between denoising and preserving boundaries from the view of quality. 

We also present quantitative results in Table~\ref{SSIM_PSNR_FFL_comparison}. Based on the bottom images from \autoref{denoising_with_real_data}, we can conclude that \verb|Topaz| contains the least noise while \verb|Noisy| contains the most noise. With this conclusion, the values in bold in the three tables show that (1) \verb|T+N| is the closest one to \verb|Topaz| besides \verb|Topaz| itself and (2) \verb|T+N| has a moderate amount of noise compared to \verb|T| and \verb|N|. This means our method is a good compromise between removing noise and preserving details, echoing with our qualitative comparison.

Besides the example in \autoref{denoising_with_real_data}, we give another example of denoising real data. From \autoref{denoising_with_real_data_zoomin_another}, we can draw the similar conclusions. \verb|Topaz| has the least noise, but compromised boundaries while \verb|T+N| has moderate amount of noise but also clearer boundaries and more visibility of spikes.

\begin{figure}[H]
\begin{center}
\includegraphics[width=\linewidth]{figures/denoising_imgs/real_data_compare/RealDataDenoising-2.png}
\caption{Denoising with real data zoom-in another example}
\label{denoising_with_real_data_zoomin_another}
\end{center}
\end{figure}

\fl{TODO: add results of reconstruction}


